Epidemiology-Aware Neural ODE with Continuous Disease Transmission Graph

Effective epidemic forecasting is critical for public health strategies and efficient medical resource allocation, especially in the face of rapidly spreading infectious diseases. However, existing deep-learning methods often overlook the dynamic nature of epidemics and fail to account for the specific mechanisms of disease transmission. In response to these challenges, we introduce an innovative end-to-end framework called Epidemiology-Aware Neural ODE with Continuous Disease Transmission Graph (EARTH) in this paper. To learn continuous and regional disease transmission patterns, we first propose EANO, which seamlessly integrates the neural ODE approach with the epidemic mechanism, considering the complex spatial spread process during epidemic evolution. Additionally, we introduce GLTG to model global infection trends and leverage these signals to guide local transmission dynamically. To accommodate both the global coherence of epidemic trends and the local nuances of epidemic transmission patterns, we build a cross-attention approach to fuse the most meaningful information for forecasting. Through the smooth synergy of both components, EARTH offers a more robust and flexible approach to understanding and predicting the spread of infectious diseases. Extensive experiments show EARTH superior performance in forecasting real-world epidemics compared to state-of-the-art methods. The code will be available at https://github.com/Emory-Melody/EpiLearn.

==> notations.tex <==


\section{Notation Table}
\label{app:notation}		
\begin{table}[h]\small
\centering
\scriptsize{\resizebox{0.9\linewidth}{!}{
\begin{tabular}{cl}
\hline
Notations & Description \\ \hline
%base
$A$ & adjacency matrix \\
$Y$ & labels of graph \\
$X$ & node featurs \\
$v_i$ & the node with indicator $i$ in graph \\
$y_i$ & label of node $v_i$\\
$A_i$ & the neighborhoods of the node $v_i$ \\
$Z$ & node-level feature, $\text{hidden dimension} \in \mathbb{R}^d$ \\ 
$U$ & output logit \\
$d$ & dimension of $z$ \\
$I$ & classes collection \\
$f$ & feature extractor \\
$g$ & classifier head \\

%method
$\mathcal{B}$ & global memory bank \\
$k$ & k-nearest neighbors in FCPP \\
$k'$ & k-nearest neighbors in global semantic graph completion \\
$c$ & prototype \\
$j$ & the index of class \\
$\omega( \cdot )$ & cosine similarity \\
$\mathbb{C}^j$ & prototypes collections \\
$w_i$ & node weight in prototype aggregation \\
$W$ & the weight sum \\
$H$ & cluster centroids num \\
$\mathbf{G}$ & the graph augmentation module \\
$F$ & hidden features in GKIC \\
$g$ & the global signal \\
$\Omega$ & probability matrix \\
$\lambda$ & the strength of augmentation \\
$\mathbf{S}$ & a Gumbel random variate \\
$\mathbb{H}$ & cross-entropy loss \\



%fed
$M$ & total number of clients \\
$m$ & the index of client \\
$P$ & distribution \\
$D^m$ & private data of the  $m$ client\\
$R$ & communication round \\
$\theta^m$ & model parameter of client $m$ \\
$E$ & local training epochs \\
% $\sigma(\cdot)$ & ReLU activation function, $\sigma(\cdot) = \max\{\cdot,0\}$ \\
$\tau$ & the parameter in contrastive method \\
$\alpha$ & the loss weight for $L_{con}$\\
$\beta$ & the loss weight for $L_{reg}$ \\
$\eta$ & learning rate  \\
\hline
\end{tabular}%
}}

\caption{Notations occurred in the paper.}
\label{tab:notation}
\end{table}
